DART: Denoising Autoregressive Transformer for Scalable Text-to-Image Generation

Diffusion models have become the dominant approach for visual generation. They are trained by denoising a Markovian process which gradually adds noise to the input. We argue that the Markovian property limits the model's ability to fully utilize the generation trajectory, leading to inefficiencies during training and inference. In this paper, we propose DART, a transformer-based model that unifies autoregressive (AR) and diffusion within a non-Markovian framework. DART iteratively denoises image patches spatially and spectrally using an AR model that has the same architecture as standard language models. DART does not rely on image quantization, which enables more effective image modeling while maintaining flexibility. Furthermore, DART seamlessly trains with both text and image data in a unified model. Our approach demonstrates competitive performance on class-conditioned and text-to-image generation tasks, offering a scalable, efficient alternative to traditional diffusion models. Through this unified framework, DART sets a new benchmark for scalable, high-quality image synthesis.

==> sections/related_work.tex <==
\section{Related Work}

==> tables/imagenet.tex <==
\begin{table}[t]
\begin{center}
\caption{Performance of \modelname{} on ImageNet 256 in comparison to baselines. }
\begin{tabular}{clcccc}
    \toprule
    % \multicolumn{6}{l}{\textbf{Class-Conditional ImageNet 256x256}} \\
    % \midrule
    Type & Model  & FID$\downarrow$ & IS$\uparrow$ & Precision$\uparrow$ & Recall$\uparrow$ \\
    % \midrule
    %GAN & GigaGAN~\citep{kang2023scaling} & 3.45 & 225.5 & 0.84 & 0.61 \\
    %GAN & StyleGAN-XL~\citep{sauer2022stylegan} & 2.30 & 265.12 & 0.78 & 0.53 \\
    \midrule
    Diff. & ADM~\citep{dhariwal2021diffusion} & 10.94 & 100.98 & 0.69 & 0.63 \\
    Diff. & CDM~\citep{ho2022cascaded} & 4.88 & 158.71 & - & - \\
    % Diff. & RIN~\citep{jabri2022scalable} & 3.42 & 182.0 & - & - \\
    Diff. & DiT~\citep{peebles2022scalable} & 2.27 & 278.24 & 0.83 & 0.57 \\
    Diff. & DiT (16 steps) \\
    %Diff. & SiT~\citep{ma2024sit}  & 2.06 &  270.27 & 0.82 & 0.59\\
    %Diff. & MaskDiT~\citep{zheng2023fast} & 2.28 &  276.56 & 0.80 & 0.61\\
    %Diff. & MDT-XL~\citep{mdt} & 1.58 & 314.73 & 0.79 & 0.65\\
    %\midrule
    %Mask. & MaskGIT~\citep{chang2022maskgit} & 6.18 & 182.1 & - & -\\
    \midrule
    AR & VQGAN~\citep{esser2021taming} & 15.78 & 74.3 & - & - \\
    AR & ViTVQ~\citep{yu2021vector} & 3.04  & 227.4 & -  & - \\
    AR & RQTran.~\citep{lee2022autoregressive} & 3.80 & 323.7 & - & - \\
    AR & VAR~\citep{tian2024visual} & 1.73 & 350.2 & 0.82 & 0.60\\
    \midrule
    Diff. + AR & MAR-L-causal~\citep{li2024autoregressive} & 19.23 & 62.3 & - & -\\
    Diff. + AR & MAR-L-bidirect~\citep{li2024autoregressive} & 3.50 & 201.4 & - & - \\
    Diff. + AR & MAR-H-bidirect~\citep{li2024autoregressive} & 1.55 & 303.7 & 0.81 & 0.62 \\
    \midrule
    Ours & \modelname{} & TBD & TBD & TBD & TBD \\
    Ours & \modelname{}-AR & TBD & TBD & TBD & TBD \\
    Ours & \modelname{}-FM & TBD & TBD & TBD & TBD \\
    \bottomrule
  \end{tabular}
  \label{tb:imagenet}
\end{center}
\end{table}

